Improving Differentiable Architecture Search with a Generative Model

In differentiable neural architecture search (NAS) algorithms like DARTS, the training set used to update model weight and the validation set used to update model architectures are sampled from the same data distribution. Thus, the uncommon features in the dataset fail to receive enough attention during training. In this paper, instead of introducing more complex NAS algorithms, we explore the idea that adding quality synthesized datasets into training can help the classification model identify its weakness and improve recognition accuracy. We introduce a training strategy called ``Differentiable Architecture Search with a Generative Model(DASGM)." In DASGM, the training set is used to update the classification model weight, while a synthesized dataset is used to train its architecture. The generated images have different distributions from the training set, which can help the classification model learn better features to identify its weakness. We formulate DASGM into a multi-level optimization framework and develop an effective algorithm to solve it. Experiments on CIFAR-10, CIFAR-100, and ImageNet have demonstrated the effectiveness of DASGM. Code will be made available.

==> figs/backup.tex <==
%%%%% V-1 Introduction



Neural architecture search (NAS) alogrithms are widely used in computer vision fields, like image classification. It can automatically search neural architecture with remarkable performance. The key idea of NAS is to build a large search space architecture and sample an optimal subset architecture from the search space. Previous research on NAS mainly uses evolution based algorithms or reinforcement learning based algorithms to sample optimal architecture. However, the computational cost of these two methods are very high. Nowadays, researchers mainly focus on developing gradient-based algorithms, which greatly reduced the computational cost by relaxing search space to be continuous and optimize the validation loss on it. Previous gradient-based algorithms are trying to design sophisticated algorithms to achieve higher accuracy while maintaining lower memory cost. However, there are several drawbacks in these algorithms: (1) gradient-based NAS algorithms suffer significant instability during training. (2) gradient-based NAS algorithms suffer heavy memory and computation overheads.  To relief these burdens, in this paper, we are interested in exploring the idea that incorporating external dataset into NAS training can help improve model performance while maintaining low memory cost. 

Our framework consists of two models: a classification model and a class-conditional GAN model. The classification model performs image classification on the images synthesised by generator. The validation loss produced by the classification model in return helps the discriminator to update its architecture. The changes in the discriminator will help generator to produce harder examples to feed into the classifier. The optimization of our framework can be summarized in four steps: (1) We first update the classification model's weight on the training set $J_1$. (2) Then, we update the class-conditional GAN's weight on the training set $J_2$. (3) Next, we update the classification model's architecture on the dataset synthesised by the generator. (4) Finally, we update the discriminator's architecture on the training dataset $J_2$. The four steps are trained end to end. Compared with traditional methods, our framework has the following highlights: (1) Our framework can be easily composed into any other NAS algorithms and help to improve architecture search performance. (2) By taking quality external dataset into training, our framework helps the classification learn better.
Besides, when class-conditional GAN and classification model are trained separately, which means we update classification model's architecture using the images generated by pre-trained generator, our framework can still achieve good performance while maintaining lower memory cost.
 
We compare our framework with Darts, P-Darts and PC-Darts and conduct experiments on CIFAR-10, CIFAR-100 and ImageNet. By comparaing the classification error and memory consumption, our framework can significantly help to improve NAS model performance. 





\begin{comment}
\section{Application to Semantic Segmentation}
In this section, we apply the generative LPT framework for semantic segmentation. Let $A$ be the architecture of a semantic segmentation model and $W$ be the network weights. The search space of $A$ follows that in \cite{liu2019autodeeplab}. $D_{ln}^{(\mathrm{tr})}$ is a semantic segmentation dataset. We train a conditional GAN which takes a segmentation map as input and generates an image. The generator is an encoder-decoder  model where the encoder takes a segmentation map as input, and the encoding is fed into the decoder to generate a corresponding image. Let $C$ denote the architecture of the encoder and $U$ denote the network weights of the encoder. The decoder and discriminator have fixed architectures (manually designed by humans). Let $V$ and $X$ denote the network weights of the decoder and discriminator. $D_{tt}^{(tr)}$ contains data pairs where the inputs are segmentation maps and outputs are images. We use the trained conditional GAN to generate semantic segmentation validation examples and use these examples to validate the semantic segmentation model. The formulation is: 
     

\begin{equation}
    \begin{array}{l}
\max _{C} \min _{A}\;\;  L\left(A, W^{*}\left(A\right), C, U^*(C), V^*(C)\right) \\
s.t. \;\;   
 U^*(C), V^*(C), X^*(C)
      =\textrm{max}_{X}\textrm{min}_{U,V} \quad L(C, U, V,X, D_{tt}^{(tr)})
\\
\quad\;\;\;
W^{*}\left(A\right)=\min _{W}\;\; L\left(A, W, D_{ln}^{(\mathrm{tr})}\right)
\end{array}
\label{eq:learning_objective}
\end{equation}
\end{comment}




%%%%%%% Validation loss version

\begin{abstract}
Previous gradient-based NAS algorithms like Darts tend to design sophisticated search algorithms to sample better model architecture from search space. However, when designing more complex algorithms, it faces severe instability during training. In this paper, instead of trying to modify NAS algorithms, we explore the idea that adding quality external datasets into training can help the classification model identify its weakness and improve model performance. 
In our framework, a class conditional GAN and a classification model are interacting with each other: the generator generates diverse samples for the classification model to train its architecture. And the validation loss from the classification model is used to update the class conditional GAN and help the generator produce better training samples. We formulate the learning by passing tests with a generative tester with a multi-level optimization framework and develop an effective algorithm to solve it. Experiments on  CIFAR-100, CIFAR-10, and ImageNet have demonstrated the effectiveness of our method.


 
\end{abstract}

\section{Introduction}
Neural architecture search (NAS) algorithms are widely used in the computer vision fields, like image classification. It can automatically search neural architecture with remarkable performances by sampling an optimal subset architecture from the search space. Due to their lower memory cost and higher accuracy, gradient-based searching algorithms are widely studied by the community. Recent models like Darts, P-Darts, and PC-darts follow similar training patterns: The search model first trains its architecture based on the training set $D_1$ and then trains its weight based on the training set $D_2$. The training set $D_1$ and $D_2$ are both randomly sampled from the training dataset. The key difference between these algorithms is more sophisticated designed tricks are added to improve training performance. The major drawback of these algorithms is the dataset used to update model architecture and the one used to update model weight follow similar distribution, which results in overfitting in the searching stage.

To relieve the burdens described above, in this paper, we are interested in exploring the idea that incorporating external datasets into NAS training can help improve model performance while maintaining low memory cost. Different from previous training patterns, we use data samples from the training set to update the model's weight and data samples synthesized by the class conditional GAN to update the model's architecture. By adding out of distribution data into training, the synthesized image samples can help the model identify its weakness during training and thus improve training accuracy. 

The training strategy is intuitively described in Figure.\ref{fig:overal}. The training set and synthesized dataset are both used to update the classification model. When training the classification model, the model's weakness will change in different iterations. Therefore, if we use a fixed synthesized dataset to update the classification model's architecture, the model will fail to identify its weakness during training. To solve this issue, we also update the class conditional GAN during training. The class conditional GAN updates its parameter and architecture based on the validation loss from the classification model and generates new image samples to feed into the training. 

In our paper, we introduce learning by passing tests with a generative tester framework to help NAS algorithms search for better architecture. We first start with second-order searching algorithms, which are more generalized in NAS algorithms. It consists of four steps: (1) We first update the classification model's weight on the training set $J_1$. (2) Then, we update the class-conditional GAN's weight on the training set $J_2$. (3) Next, we update the classification model's architecture on the dataset synthesized by the generator. (4) Finally, we update the discriminator's architecture on the training dataset $J_2$. The four steps are trained end-to-end. Then, we introduce a reduced framework for first-order searching algorithms, which are more widely used in recent NAS algorithms like PC-Darts. In the reduced framework, the training steps are similar to the original framework but we only search the classification model's architecture.



%Compared with traditional methods, our framework has the following highlights: (1) Our framework can be easily composed into any other NAS algorithms and help to improve architecture search performance. (2) By taking quality external dataset into training, our framework helps the classification learn better. We compare our framework with Darts, P-Darts and PC-Darts and conduct experiments on CIFAR-10, CIFAR-100 and ImageNet. By comparaing the classification error and memory consumption, our framework can significantly help to improve NAS model performance. 

%Besides, when class-conditional GAN and classification model are trained separately, which means we update classification model's architecture using the images generated by pre-trained generator, our framework can still achieve good performance while maintaining lower memory cost. 
\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figs/illu.pdf}
	\caption{Illustration of learning by tests with a generative tester. Different from traditional gradient-based NAS approaches, which propose sophisticatedly designed search algorithms to sample better search space, we incorporate external dataset generated by class-conditional GAN into searching and achieve better performance.
	}  
	\label{fig:overal}
\end{figure}


The following are the key contributions of our work: 

\begin{itemize}
    \item For the first time, we incorporate external dataset to gradient-based NAS training and significantly improves model performance on CIFAR-100, CIFAR-10, and ImageNet. 
    \item We propose a multi-level optimization framework to formulate learning by passing tests with a generative tester and developed an algorithm to solve it.
    \item Our approach can be generalized into any gradient-based NAS approaches. Experiments on Darts, P-darts and PC-darts have demonstrated the effectiveness of our method.
\end{itemize}


\section{Related Works}
\subsection{Neural Architecture Search}
Neural architecture search (NAS) aims at automatically searching neural architecture with better performance in machine learning tasks. Compared with traditional manually designed models, NAS can save more time and achieve better performance. Existing NAS methods can be categorized into three groups: (1) reinforcement learning-based approaches ~\cite{zoph2016neural,pham2018efficient,zoph2018learning} (2) evolution-based approaches ~\cite{liu2017hierarchical,real2019regularized}, and (3) gradient-based approaches ~\cite{cai2018proxylessnas,liu2018darts,xie2018snas}.

For reinforcement learning-based approaches, NAS models sample candidate architectures from search space based on reinforcement learning algorithms. For evolution-based approaches, candidate architectures are represented as a population. Highly-performing architectures are allowed to generate offspring while poorly-performing architectures are eliminated. For gradient-based approaches, the search space is relaxed to be continuous and optimized based on its validation loss by gradient descent. The first two approaches take expensive computational costs to train a NAS model(1800 GPU days for reinforcement learning-based approaches and 3150 GPU days for evolution-based approaches). Nowadays, due to its low search cost, research on NAS mainly focuses on proposing better gradient-based algorithms to sample from search space.

Previous research like GTN~\cite{pmlr-v119-such20a} also tried to use generative models to accelerate neural architecture search. But we have two major differences: (1) GTN mainly accelerates evolution-based NAS approaches, while our work focuses on gradient-based approaches. (2) GTN only updates the generator during training, while our work updates the discriminator's architecture and both the generator and the discriminator's weight. To the best of our knowledge, we are the first to incorporate external datasets in gradient-based NAS and the algorithm can be generalized to any other gradient-based NAS approaches.




\subsection{Generative Adversarial Networks}
GANs~\cite{DBLP:journals/corr/GoodfellowPMXWOCB14} aims at synthesizing images from random vectors. A generator is used to map random vectors to synthesized images and a discriminator is used to 
distinguish generated images from real images. Class conditional GANs~\cite{DBLP:journals/corr/MirzaO14,pmlr-v70-odena17a} mainly focus on generating high quality images from class labels in large dataset. There are mainly three approaches to improve image generation quality: (1) design more complex network architectures for generator and discriminator (2) introduce better training strategies and (3) design more sophisticated loss functions. 

For example, BigGAN\cite{DBLP:conf/iclr/BrockDS19} applied orthogonal regularization to the generator and can synthesis high-resolution images on large datasets like ImageNet. SAGAN\cite{zhang2019self} introduced a self-attention mechanism into convolutional GANs to help model long-range, multi-level dependencies across image regions. StyleGAN\cite{DBLP:journals/corr/abs-1812-04948} borrowed network architecture from style transfer networks and enables intuitive, scale-specific control of image synthesis.  In this paper, we employ class conditional GANs to generate images as the external dataset to train gradient-based NAS models in the search stage. 



%\subsection{Learning by Passing Tests}
%Learning by passing tests(LPT) borrows the learning methodology from human to improve image classification accuracy. The framework consists of two parts: a tester and a learner. The tester creates test samples with different levels of difficulty, while the learner takes the test samples into training and identify its weakness in learning. In our paper, the learner is the classification model and the tester is the class-conditional GAN. Compared with previous LPT models, we have the following improvements: (1) Instead of selecting training samples from the validation set, we use a generator to generate images. Previous test samples 
%can only be selected from the validation set and the sample may not be difficult enough for the classification model to train. (2) When the models are trained separately, we can use a pre-trained model to generate images. It can greatly reduce the memory consumption while not reducing too much model performance.
\subsection{Multi level Optimization}

Multi-level optimization is defined as a mathematical program, where an optimization problem contains another optimization problem as a constraint. It has wide applications in machine learning, supply chain, and electricity. The problem consists of two-level optimization tasks: upper level and lower level. The two optimization tasks have different constraints, objectives, and decision vectors. When solving the multi-level optimization problems, the lower level is a parametric optimization problem solved based on lower-level constraints and upper-level decision vectors. The lower-level optimization problems also serve as constraints to upper-level optimization problems. The optimization results are the vectors with lower-level optimal and satisfy upper-level constraints.
In our paper, we use a decent method to solve the optimization problem by giving a descent direction in the upper-level function while keeping the lower-level function at an optimal position.

\section{Problem Formulation}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/overal.pdf}
  \caption{Overview of our framework. Firstly, we update the classification model's weight on the training set $J_1$. Then, we update the class-conditional GAN's weight on the training set $J_2$. Next, we update the classification model's architecture on the dataset synthesised by the generator. Finally, we update the discriminator's architecture on the training dataset $J_2$.}
    \label{fig:fm}
\end{figure*}

\paragraph{Overview.} Two models are interacting with each other in our framework: a classification model and a class-conditional GAN model. The two models interact with each other to achieve better classification performance. The class-conditional GAN's generator generates diverse examples to help the classification model search for better architecture. The class-conditional GAN updates its discriminator's architecture based on the classification model's validation loss. The updated discriminator can in return help the generator generates better examples to feed into the classification model .

As shown in Figure.\ref{fig:fm}, our model consists of four stages: In the first stage, the classification model trains its network weights $W$ on the training set $J_1$ with the architecture fixed; In the second stage, the class-conditional GAN model trains its network weights $G$ and $E$ on the training set $J_2$ with the architecture fixed; In the third stage, the classification model updates its architecture on the dataset $J_3$ created by the class-conditional GAN model; In the fourth stage, the discriminator updates its architecture $B$ on the created dataset $J_2$. All four stages are trained end-to-end. The notions are summarized in Table. \ref{tb:notations}.

\begin{table}[h]
\centering
\begin{tabular}{l|l}
\hline
Notation & Meaning \\
\hline
$A$ & Architecture of the classification model\\
$W$ & Network weights of the classification model\\
$G$ & Network weights of the generator \\
$B$ & Architecture of the discriminator \\
$E$ & Network weights of the discriminator \\
$J_1$ & Training data set I\\
$J_2$ & Training data set II\\
$J_3$ & Images generated by generator  \\
\hline
\end{tabular}
\caption{Notations}
\label{tb:notations}
\end{table}

\paragraph{Objective.} 
In the framework described above, during training, the classification model aims at minimize the classification loss and the class-conditional GAN model aims at minimize the generator loss while maximize the discriminator loss. When the models are interacting with each other, we aim at minimize the overall loss by adjusting the architecture of the classification model and maximize the overall loss by adjusting the architecture of the discriminator.

Putting all the objective functions described above together, we get the following optimization framework:


\begin{equation}
    \begin{array}{l}
\max _{B} \min _{A}\;\;  L_{overal}\left(A, W^{*}\left(A\right), G^*(B)\right) \\
s.t. \;\;   
 G^*(B)
      =\textrm{argmin}_{G}\textrm{argmax}_{E} \quad L_{GAN}(B, G, E,J_2)
\\
\quad\;\;\;
W^{*}\left(A\right)=\textrm{argmin} _{W}\;\; L_{class}\left(A, W, J_1\right)
\end{array}
\label{eq:learning_objective}
\end{equation}

where $L_{class}\left(A, W, J_1\right)$ is the classification loss and $L_{GAN}(B, G, E,J_2)$ is the class-conditional GAN loss. $J_1$ and $J_2$ are both  training set containing class-image pairs, which correspond to the dataset $J_1$ and $J_2$.
Given $G^*(B)$, it is used to generate a synthetic validation dataset $J_3$, which is used to evaluate the classification model's performance. In $\max _{B} \min _{A}\;\;  L_{overal}\left(A, W^{*}\left(A\right), G^*(B)\right)$, the classification model aims at maximizing the validation loss by adjusting $A$ and the class-conditional GAN model aims at maximizing the validation loss by adjusting $B$. 

The the optimization problems described above correspond to the four learning stages in Figure.\ref{fig:fm}. From bottom to up, the first two optimization problems correspond to the first two stages. The third optimization problem corresponds to the third and fourth stages. The four stages are performed jointly end-to-end in a multi-level optimization framework, where different stages influence each other. The solution $W(A)^{*}$ is obtained by minimizing the training loss $L_{class}\left(A, W, J_1\right)$. The solution $G^*(B)$ is obtained by adjusting $E$ to minimize the training loss $L_{GAN}(B, G, E, J_2)$ and adjusting $G$ to maximize the training loss $L_{GAN}(B, G, E, J_2)$. The obtained $W(A)^{*}$ and $G^*(B)$ are nested on the constraint of the third optimization problem.  The $G^*(B)$ in the second stages is used to generate the augmented dataset $J_3$ to update the classification model architecture in the third optimization problem. 



%The tester is a conditional GAN model, which takes a class label as input and generates an image belonging to this class. It is composed of a generator and discriminator. The generator has a fixed architecture (designed by humans) and learnable network weights $G$. The discriminator has a learnable architecture $B$ and learnable network weights $E$. 

%The training process can be summarized into four stages. The four stages are performed jointly end-to-end in a multi-level optimization framework, where different stages influence each other.

%\begin{itemize}
%    \item In the first stage, the learner trains its network weights on the training set of task J1 with the architecture fixed.
%    \item In the second stage, the tester trains its generator and discriminator on a created test to perform the target task J2, with the architecture fixed.
%    \item In the third stage, the learner updates its model architecture by minimizing the predictive loss L on the test created by the tester
%    \item In the fourth stage, the tester updates its discriminator architecture by maximizing L on the validation set of J2.
%\end{itemize}

\section{Optimization Algorithm}
In this section, we develop a gradient-based optimization algorithm to solve the learning by passing tests with a generative tester problem. Firstly, we update the generator, the discriminator, and the classification model's weight in every minibatch. We approximate $W^{*}(A)$ using one-step gradient descent w.r.t $L_{class}\left(A, W, J_1\right)$, where $\eta_{w}$ is the learning rate:

\begin{equation}
\label{eq:learner}
    W^{*}(A)=W'=W-\eta_{W} \nabla_{w} L_{class}\left(A, W, J_1\right). 
\end{equation}

For $G^*(B)$, we approximate it using one-step gradient ascent w.r.t $L_{GAN}(B, G, E, J_2)$, where $\eta_{g}$ is the learning rate:
\begin{equation}
\label{eq:generator}
    G^*(B)=G'=G+\eta_{g}\nabla_{G}L_{GAN}(B, G, E, J_2).
\end{equation}

We update discriminator's weight $E$ using one-step gradient descent, where $\eta_{e}$ is the learning rate:
\begin{equation}
\label{eq:discriminator_loss}
    E\gets E-\eta_{e}\nabla_{E}L_{GAN}(B, G, E, J_2).
\end{equation}

We plug updated classification model weight $W'$ and updated generator weight $G'$ into objective function $L_{overal}\left(A, W^{*}\left(A\right), G^*(B)\right)$ and get an approximated objective: $L\left(A, W', G'\right)$. We update classification model's architecture $A$ using gradient descent, where $\eta_a$ is the learning rate:

\begin{equation}
\label{eq:learn_archi}
    A\gets A-\eta_a\nabla_{A}L_{overal}\left(A, W', G'\right),
\end{equation}

where

\begin{equation}
\begin{array}{l}
\label{eq:learn_expand1}
    \nabla_{A}L_{overal}\left(A, W', G'\right) = \\
    \nabla_{A}L_{overal}\left(A, W-\eta \nabla_{W} L_{class}\left(A, W, J_1\right), G'\right) = \\
    \nabla_{A} L_{overal}\left(A, W^{\prime}, G^{\prime}\right)-
    \eta \nabla_{A, W}^{2} L_{class}\left(A, W, J_1\right) \\ \nabla_{W^{\prime}} L_{overal}\left(A, W^{\prime}, G^{\prime}\right)
\end{array}
\end{equation}

The second term in the third line involves expensive matrix-vector product, whose computational complexity can be reduced by a finite difference approximation:

\begin{equation}
\begin{array}{l}
\label{eq:learn_expand2}
\nabla_{A, W}^{2} L_{class}\left(A, W, J_1\right) \nabla_{W^{\prime}} L_{overal}\left(A, W^{\prime}, G^{\prime}\right)  \approx  \\
\frac{1}{2 \alpha_{\ln }} \left(\nabla_{A} L_{class}\left(A, W^{+}, J_1\right)-\nabla_{A} L_{class}\left(A, W^{-}, J_1\right)\right)
\end{array}
\end{equation}

where $W^{\pm}=W \pm \alpha \nabla_{W^{\prime}} L_{overal}\left(A, W^{\prime}, G^{\prime}\right)$ and $\alpha_{\ln }$ is a small scalar that equals $0.01 /\left\|\nabla_{W^{\prime}} L_{overal}\left(A, W^{\prime},  G^{\prime}\right)\right\|_{2}$

and update discriminator's architecture $B$ using gradient ascent, , where $\eta_b$ is the learning rate:
\begin{equation}
\label{eq:dis_archi}
    B\gets B+\eta_b\nabla_{B}L_{overal}\left(A, W', G'\right).
\end{equation}


where
\begin{equation}
\begin{array}{l}
\label{eq:dis_expand1}
    \nabla_{B}L\left(A, W', G'\right) = \frac{\partial G'}{\partial B} \frac{\partial L_{overal}\left(A, W', G'\right)}{\partial G'} \\
    = \eta_g \nabla_{B,G}^{2}L_{GAN}(B, G, E, J_2)\nabla_{G'}L_{overal}\left(A, W', G'\right)
    
    
    %\nabla_{B}L\left(A, W', G+\eta\nabla_{G}L(B, G, E,D_{tt}^{(tr)})\right) \\
   % =\nabla_{B}L\left(A, W', G\right) + \nabla_{B}L\left(A, W', \eta\nabla_{G}L(B,E,D_{tt}^{(tr)})\right) \\
    %= \frac{\partial G}{\partial B} \frac{\partial L\left(A, W', G\right)}{\partial G}  + \eta\frac{\partial G}{\partial B}  \frac{\partial L\left(A, W', \nabla_{G}L(B,E,D_{tt}^{(tr)})\right)}{\partial G} 
\end{array}
\end{equation}


The term in the second line involves expensive matrix-vector product, whose computational complexity can be reduced by a finite difference approximation:
\begin{equation}
\begin{array}{l}
\label{eq:dis_expand2}
\nabla_{B}L_{overal}\left(A, W', G'\right) \approx \\
\frac{1}{2 \eta_g }\left(\nabla_{B} L_{GAN}\left(B, G^{+}, E, J_2\right)-\nabla_{B} L_{GAN}\left(B, G^{-},  E, J_2\right)\right)

\end{array}
\end{equation}

where $G^{\pm}=G \pm \alpha \nabla_{G^{\prime}} L_{overal}\left(A, W^{\prime}, G^{\prime}\right)$ and $\eta_g$ is a small scalar that equals $0.01 /\left\|\nabla_{G^{\prime}} L_{overal}\left(A, W^{\prime},  G^{\prime}\right)\right\|_{2}$

The overall algorithm is summarized in Algorithm~\ref{alg:opt}. 

\begin{algorithm}[h]
\caption{Optimization algorithm for LPT with a generator}
\label{alg:opt}
%\SetAlgoLined
\begin{algorithmic}
\While{not converged}
  \State Update classifier architecture using Eq.(\ref{eq:learn_archi})
  \If{second order approximation}
    \State Update discriminator architecture using Eq.(\ref{eq:dis_archi})
    
  \EndIf 
  \State Update classifier weight using Eq.(\ref{eq:learner})
  \State Update generator weight using Eq.(\ref{eq:generator})
  \State Update discriminator weight using Eq.(\ref{eq:discriminator_loss})
\EndWhile 
\end{algorithmic}
\end{algorithm}

\paragraph{First-order approximation}
The second-order approximation is used in gradient-based NAS approaches like Darts. However, in most recent papers, first-order approximation algorithms are applied to speed up training. By applying our framework to these algorithms, we found the model performance can be greatly improved if we only update the class conditional GAN's weight. On the contrary, if we update both the classification model's architecture and the discriminator's architecture, the classification accuracy is reduced. This is partly because, in the first-order approximation, we assume $W^{*}(A)$ is the same as $W$ when optimizing the validation loss. If we search for both the classification model's architecture and the discriminator's architecture, the search space is much smaller and we might fall into a local minimum.

Therefore, we also introduce a reduced framework consisting of three stages when first-order approximation is applied: In the first stage, the classification model trains its network weights $W$ on the training set $J_1$ with the architecture fixed; In the second stage, the class-conditional GAN model trains its network weights $G$ and $E$ on the training set $J_2$ with the architecture fixed; In the third stage, the discriminator updates its architecture $B$ on the created dataset $J_2$.
